GAN-Control: Explicitly Controllable GANs

We present a framework for training GANs with explicit control over generated images. We are able to control the generated image by settings exact attributes such as age, pose, expression, etc. Most approaches for editing GAN-generated images achieve partial control by leveraging the latent space disentanglement properties, obtained implicitly after standard GAN training. Such methods are able to change the relative intensity of certain attributes, but not explicitly set their values. Recently proposed methods, designed for explicit control over human faces, harness morphable 3D face models to allow fine-grained control capabilities in GANs. Unlike these methods, our control is not constrained to morphable 3D face model parameters and is extendable beyond the domain of human faces. Using contrastive learning, we obtain GANs with an explicitly disentangled latent space. This disentanglement is utilized to train control-encoders mapping human-interpretable inputs to suitable latent vectors, thus allowing explicit control. In the domain of human faces we demonstrate control over identity, age, pose, expression, hair color and illumination. We also demonstrate control capabilities of our framework in the domains of painted portraits and dog image generation. We demonstrate that our approach achieves state-of-the-art performance both qualitatively and quantitatively.

==> comparison_to_end_to_end_training.tex <==
\subsection{Comparison with training end-to-end (two-phase vs. one-phase)}
\label{sec:e2e_comparison}
% We believe that training the pipeline in two phases has multiple benefits: each phase is simpler, and a disentangled GAN even without explicit control is beneficial in its own right.
% However, training in two phases can potentially be more complex than training a single network end-to-end.
In this section we explore an alternative approach to the one presented in the main paper in which rather than training the model using two phases, we use a single phased, end-to-end approach.
This is to highlight the benefits of our proposed method.

The end-to-end model is trained in a single training phase. In every iteration the inputs to the models are control attribute values ($y^k$) rather than latent vectors. For every attribute (except for the ID and \textit{other}) a matching loss is used to penalize the disagreement between the input control value and the output image. 
The attribute values of the generated image are predicted using the pre-trained models (the same ones as in our two-phase approach) and are compared to the input control values for measuring the disagreement.
For the ID preservation we used the original contrastive terms as in the main paper (Sec. 3.1). The reason for this is that penalizing for the ID disagreement as done for all other attributes (via a matching loss) requires to allocate a fixed set of IDs which will limit the framework.
An additional reason for not using an ID matching loss is that the task of defining a control for an ID is more complicated than for other attributes.
The architecture of the end-to-end model is the same as the final architecture we use for inference after the second training phase of our original approach (see architecture under \textit{inference} in Figure 2 of the main paper).
We derive a feasible set of input attribute control values based on the ones inferred from the actual samples in the FFHQ dataset. 
Practically for each image in the FFHQ dataset (70K images) we extract all its attributes via the pre-trained predictors, resulting in five attribute datasets of size 70K each (corresponding to pose, expression, illumination, age and hair color).
\input{figures/fig_ours_vs_e2e_ori}
\input{figures/fig_ours_vs_e2e_age}
\input{figures/fig_ours_vs_e2e_exp}
\input{figures/fig_ours_vs_e2e_gam}
\input{figures/fig_ours_vs_e2e_hai}
\input{tabels/table_ours_vs_end2end}

We experimented with several options of training such an end-to-end approach. The options vary in the different weight configurations of the matching loss terms and scheduling mechanisms (all training runs that used the matching loss starting from the first iteration diverged after a few iterations).
Here we present results of two models trained end-to-end, both used the matching loss starting from the 20K's iteration (when the generated images start to resemble faces).
We used two configurations of weights where for the first model (End2End) the weights are 10 times smaller in magnitude than for the second one (End2End-10x).
In Table~\ref{tab:table_end2end} we present the comparison of the control precision (similar to Table 3 in the main paper), ID preservation (similar to Table 4 in the main paper) and FID for the two end-to-end models and our two-phased model (Ours).
In the rightmost column we present the FFHQ statistics as a baseline (no control).
As evident from the table, our original two-phased model achieves significantly better results across all metrics.
As expected, the E2E-10x model achieves better control precision than the E2E model at the expense of reduced photorealism (FID score) and ID preservation.
However, at both ends of the spectrum the results are inferior to those achieved by our two-phased model.
We also demonstrate this qualitatively in Figures~\ref{fig:end2end_ori},~\ref{fig:end2end_age},~\ref{fig:end2end_exp},~\ref{fig:end2end_gamma} and ~\ref{fig:end2end_hair}.

==> dog_generation.tex <==
\subsection{Dog generation}
In this experiment we aim to control the identity and pose of dogs, to demonstrate our capability to generalize to additional domains other than human faces.

%\paragraph{Implementation Details}
\textbf{Implementation details:} We use AFHQ~\cite{choi2020starganv2}, 5,239 dog face images downsampled to 512x512 resolution. 
We use StyleGAN2 with non-leaking augmentation~\cite{karras2020training} as before, for paintings.
For preserving dog IDs we use two different models ($M_{ID}^0$, $M_{ID}^1$).
% For preserving dogs IDs we use two different losses.
% For preserving dogs IDs we use two $l_{id}$ losses, both with properties aiming to preserve identities of dogs.
$M_{ID}^0$ is a dog-face recognition model DogFaceNet~\cite{10.1007/978-3-030-29894-4_34}.
We noticed that DogFaceNet often recognizes two dogs to be the same if a similar pattern is present on their heads, even if they are of different breeds.
To overcome this issue, we use ResNet18~\cite{He2016DeepRL} trained on ImageNet~\cite{imagenet_cvpr09} as $M_{ID}^1$ (the penultimate layer is used for the distance comparison). 
We use this model since of the 1K classes in the ImageNet challenge, 90 are dog-breeds.
% We use an ImageNet model having 90 dog-breeds out of the 1K classes it was trained on.
% Using $M_{id}^1$ is penalized harder for generating two "same" dogs from different breeds.
For $M_{pose}$ we use the same pose detection network as for human faces and paintings~\cite{Ruiz_2018_CVPR_Workshops}. 
% Surprisingly, it does a fair job on dog faces. 

%\paragraph{Quantitative evaluation}
\textbf{Photorealism:}
The FID scores are $8.74$ and $8.22$ for our controlled and for the baseline models, respectively.

%\paragraph{Qualitative evaluation}
\textbf{Qualitative evaluation:} 
Fig.~\ref{fig:afhq_orientation_control} shows precise control over dog pose using $E_{pose}$.
We show that the pose estimation network was able to provide enough guidance to the GAN even though the domain gap between dog and human faces is quite large.
Since dogs are rarely photographed from below, our model was not able to generate images of dogs with a positive pitch.
Unlike humans, dogs exhibit a large variability in head-roll, therefore the model was able to capture this aspect well.

\input{figures/fig_afhq_orientation}

==> figures/fig_afhq_orientation.tex <==
\begin{figure}[]
%\centering
\newcolumntype{Y}{>{\centering\arraybackslash}X}

\setlength{\tabcolsep}{0pt}
\begin{tabular}{c}
    \footnotesize
    \begin{tabularx}{\linewidth}{ Y Y Y Y Y }
    Yaw$=\!30\degree$ & 
    $\!15\degree$ &
    $\!0\degree$ &
    $\!-15\degree$ & 
    $\!-30\degree$
    \end{tabularx}

    \\
    \includegraphics[width=0.98\linewidth]{images/afhq/0orientation_0002.jpg} \\
    %\includegraphics[width=0.98\linewidth]{latex/images/afhq/0orientation_0006.jpg} \\
    %\includegraphics[width=0.98\linewidth]{latex/images/afhq/0orientation_0012.jpg} \\
    %\includegraphics[width=0.98\linewidth]{latex/images/afhq/0orientation_0018.jpg} \\
    %\includegraphics[width=0.98\linewidth]{latex/images/afhq/0orientation_0019.jpg} \\
    \footnotesize
    \begin{tabularx}{\linewidth}{ Y Y Y Y Y }
    Roll$=\!20\degree$ & 
    $\!-20\degree$ &
    $\!0\degree$ &
    Pitch$=\!-10\degree$ & 
    $\!-20\degree$
    \end{tabularx}
    \\
    \includegraphics[width=0.98\linewidth]{images/afhq/1orientation_0023.jpg} \\
\end{tabular}
\vspace{-0.2cm}
\caption{\textbf{Controlling head pose in dog images:} Generation results using $E_{pose}$.}
\label{fig:afhq_orientation_control}
\end{figure}

==> figures/fig_age_control.tex <==
\begin{figure}[htbp!]
%\centering
\newcolumntype{Y}{>{\centering\arraybackslash}X}

\setlength{\tabcolsep}{0pt}
\begin{tabular}{c}
    \footnotesize
    \begin{tabularx}{0.98\linewidth}{ Y Y Y Y Y }
    Age$=\!15$yo & 
    $30$yo &
    $45$yo &
    $60$yo & 
    $75$yo
    \end{tabularx}
    \\
    %\includegraphics[width=0.98\linewidth]{latex/images/ffhq/ages/age_0001_chosen.jpg} \\
    %\includegraphics[width=0.98\linewidth]{latex/images/ffhq/ages/age_0002_chosen.jpg} \\
    \includegraphics[width=0.98\linewidth]{latex/images/ffhq/ages/age_0003_chosen.jpg} \\
    \includegraphics[width=0.98\linewidth]{latex/images/ffhq/ages/age_0029_chosen.jpg} \\
    %\includegraphics[width=0.98\linewidth]{latex/images/ffhq/ages/age_0006_chosen.jpg} \\
    \includegraphics[width=0.98\linewidth]{latex/images/ffhq/ages/age_0009_chosen.jpg} \\
    %\includegraphics[width=0.98\linewidth]{latex/images/ffhq/ages/age_0018_chosen.jpg} \\
    %\includegraphics[width=0.98\linewidth]{latex/images/ffhq/ages/age_0020_chosen.jpg} \\
    %\includegraphics[width=0.98\linewidth]{latex/images/ffhq/ages/age_0022_chosen.jpg} \\
    %\includegraphics[width=0.98\linewidth]{latex/images/ffhq/ages/age_0023_chosen.jpg} \\
\end{tabular}
\vspace{-0.2cm}
\caption{\textbf{Controlling age:} Generation results using $E_{age}$ for controlling age.}
\label{fig:age_control}
\end{figure}

==> figures/fig_ori_exp_age_gamma.tex <==
\begin{figure*}[t]
%\centering
\newcolumntype{Y}{>{\centering\arraybackslash}X}

\begin{tabular}{c c}
    %\rotatebox{90}{\hspace{9.5mm}{Orientation\textcolor{white}{p}}}
    Orientation & Orientation+Expression \\
    \includegraphics[width=0.4\linewidth]{latex/images/ffhq/ori_exp_age_gamma/ori.jpg} &
    %\rotatebox{90}{\hspace{9.5mm}{Orientation+Expression\textcolor{white}{p}}}
    \includegraphics[width=0.4\linewidth]{latex/images/ffhq/ori_exp_age_gamma/ori_exp.jpg} \\
     Orientation+Expression+Age & Orientation+Expression+Age+Illumination \\
    \includegraphics[width=0.4\linewidth]{latex/images/ffhq/ori_exp_age_gamma/ori_exp_age.jpg} &
    \includegraphics[width=0.4\linewidth]{latex/images/ffhq/ori_exp_age_gamma/ori_exp_age_gam.jpg}
\end{tabular}

\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{0.2}
\begin{tabular}{c | c}
    %\begin{tabular}{c c}
    %    & \rotatebox{90}{{Target}} \\
    %    Source & \\
    %\end{tabular}
    \includegraphics[width=0.08\linewidth]{latex/images/ffhq/ori_exp_age_gamma/st.png}
    &
    \includegraphics[width=0.32\linewidth]{latex/images/ffhq/ori_exp_age_gamma/target.jpg}
    \\
    \hline
    
    \includegraphics[width=0.08\linewidth]{latex/images/ffhq/ori_exp_age_gamma/source.jpg}
    &
    \includegraphics[width=0.32\linewidth]{latex/images/ffhq/ori_exp_age_gamma/ori0.jpg}
\end{tabular}
\vspace{-0.2cm}
\caption{\textbf{Disentanglement ablation study:} \alon{tried something - this is going to be in the supplementary}}
\label{fig:disentanglement_ablation_study}
\end{figure*}

==> figures/fig_orientation_control.tex <==
\begin{figure}[htbp!]
%\centering
\newcolumntype{Y}{>{\centering\arraybackslash}X}

\setlength{\tabcolsep}{0pt}
\begin{tabular}{c}
    \footnotesize
    \begin{tabularx}{\linewidth}{ Y Y Y Y Y }
    Yaw$=\!30\degree$ & 
    $\!15\degree$ &
    $\!0\degree$ &
    $\!-15\degree$ & 
    $\!-30\degree$
    \end{tabularx}
    \\
    \includegraphics[width=0.98\linewidth]{latex/images/ffhq/ori/orientation_0002_chosen.jpg} \\
    \footnotesize
    \begin{tabularx}{\linewidth}{ Y Y Y Y Y }
    Pitch$=\!20\degree$ & 
    $\!10\degree$ &
    $\!0\degree$ &
    $\!-10\degree$ & 
    $\!-20\degree$
    \end{tabularx}
    \\
    \includegraphics[width=0.98\linewidth]{latex/images/ffhq/ori/uorientation_0031_chosen.jpg} \\
\end{tabular}
\vspace{-0.2cm}
\caption{\textbf{Controlling head pose:} Generation results using $E_{pose}$ for controlling head orientation pitch and yaw (in degrees).}
\label{fig:orientation_control}
\end{figure}

==> figures/fig_ours_vs_e2e_age.tex <==
\begin{figure}[]
%\centering
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1}

\begin{tabular}{c}
    \footnotesize
    \hspace{4mm}\begin{tabularx}{0.9\linewidth}{ Y Y Y Y Y }
    Age=$15$yo &
    $30$yo &
    $45$yo &
    $60$yo &
    $75$yo
    \end{tabularx}
    \\
    \rotatebox{90}{
    \begin{tabularx}{0.36\linewidth}{ Y }
        \footnotesize
        E2E
    \end{tabularx}}
    \includegraphics[width=0.9\linewidth]{images/end2end_comp/age/e2e.jpg}
    \\
    \rotatebox{90}{
    \begin{tabularx}{0.36\linewidth}{ Y }
        \footnotesize
        E2E-10x
    \end{tabularx}}
    \includegraphics[width=0.9\linewidth]{images/end2end_comp/age/e2e10x.jpg}
    \\
    \rotatebox{90}{
    \begin{tabularx}{0.36\linewidth}{ Y }
        \footnotesize
        \textbf{Ours}
    \end{tabularx}}
    \includegraphics[width=0.9\linewidth]{images/end2end_comp/age/ours.jpg}
    \\
    
\end{tabular}

\caption{\textbf{Ours vs. end-to-end age control}}
\label{fig:end2end_age}
\end{figure}

==> figures/fig_ours_vs_e2e_exp.tex <==
\begin{figure}[]
%\centering
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1}

\begin{tabular}{c}
    \footnotesize
    \hspace{4mm}\begin{tabularx}{0.9\linewidth}{ Y Y Y Y Y }
    Exp. $1$ &
    Exp. $2$ &
    Exp. $3$ &
    Exp. $4$ &
    Exp. $5$
    \end{tabularx}
    \\
    \rotatebox{90}{
    \begin{tabularx}{0.36\linewidth}{ Y }
        \footnotesize
        E2E
    \end{tabularx}}
    \includegraphics[width=0.9\linewidth]{images/end2end_comp/exp/e2e.jpg}
    \\
    \rotatebox{90}{
    \begin{tabularx}{0.36\linewidth}{ Y }
        \footnotesize
        E2E-10x
    \end{tabularx}}
    \includegraphics[width=0.9\linewidth]{images/end2end_comp/exp/e2e10x.jpg}
    \\
    \rotatebox{90}{
    \begin{tabularx}{0.36\linewidth}{ Y }
        \footnotesize
        \textbf{Ours}
    \end{tabularx}}
    \includegraphics[width=0.9\linewidth]{images/end2end_comp/exp/ours.jpg}
    \\
    
\end{tabular}

\caption{\textbf{Ours vs. end-to-end expression control}}
\label{fig:end2end_exp}
\end{figure}

==> figures/fig_ours_vs_e2e_gam.tex <==
\begin{figure}[]
%\centering
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1}

\begin{tabular}{c}
    \footnotesize
    \hspace{4mm}\begin{tabularx}{0.9\linewidth}{ Y Y Y Y Y }
    Illum. $1$ &
    Illum. $2$ &
    Illum. $3$ &
    Illum. $4$ &
    Illum. $5$
    \end{tabularx}
    \\
    \rotatebox{90}{
    \begin{tabularx}{0.36\linewidth}{ Y }
        \footnotesize
        E2E
    \end{tabularx}}
    \includegraphics[width=0.9\linewidth]{images/end2end_comp/gam/e2e.jpg}
    \\
    \rotatebox{90}{
    \begin{tabularx}{0.36\linewidth}{ Y }
        \footnotesize
        E2E-10x
    \end{tabularx}}
    \includegraphics[width=0.9\linewidth]{images/end2end_comp/gam/e2e10x.jpg}
    \\
    \rotatebox{90}{
    \begin{tabularx}{0.36\linewidth}{ Y }
        \footnotesize
        \textbf{Ours}
    \end{tabularx}}
    \includegraphics[width=0.9\linewidth]{images/end2end_comp/gam/ours.jpg}
    \\
    
\end{tabular}

\caption{\textbf{Ours vs. end-to-end illumination control}}
\label{fig:end2end_gamma}
\end{figure}

==> figures/fig_ours_vs_e2e_hai.tex <==
\begin{figure}[]
%\centering
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1}

\definecolor{color1}{rgb}{0.1077, 0.0810, 0.0682}
\definecolor{color2}{rgb}{0.2358, 0.1874, 0.1546}
\definecolor{color3}{rgb}{0.3892, 0.2731, 0.1709}
\definecolor{color4}{rgb}{0.6373, 0.5166, 0.3736}
\definecolor{color5}{rgb}{0.7670, 0.6083, 0.5103}

\begin{tabular}{c}
    \footnotesize
    \hspace{4mm}\begin{tabularx}{0.9\linewidth}{ Y Y Y Y Y }
    \textcolor{color1}{\textbf{\hspace{4mm}Color $\pmb{1}$}} &
    \textcolor{color2}{\textbf{\hspace{4mm}Color $\pmb{2}$}} &
    \textcolor{color3}{\textbf{\hspace{4mm}Color $\pmb{3}$}} &
    \textcolor{color4}{\textbf{\hspace{4mm}Color $\pmb{4}$}} &
    \textcolor{color5}{\textbf{\hspace{4mm}Color $\pmb{5}$}}
    \end{tabularx}
    \\
    \rotatebox{90}{
    \begin{tabularx}{0.36\linewidth}{ Y }
        \footnotesize
        E2E
    \end{tabularx}}
    \includegraphics[width=0.9\linewidth]{images/end2end_comp/hai/e2e.jpg}
    \\
    \rotatebox{90}{
    \begin{tabularx}{0.36\linewidth}{ Y }
        \footnotesize
        E2E-10x
    \end{tabularx}}
    \includegraphics[width=0.9\linewidth]{images/end2end_comp/hai/e2e10x.jpg}
    \\
    \rotatebox{90}{
    \begin{tabularx}{0.36\linewidth}{ Y }
        \footnotesize
        \textbf{Ours}
    \end{tabularx}}
    \includegraphics[width=0.9\linewidth]{images/end2end_comp/hai/ours.jpg}
    \\
    
\end{tabular}

\caption{\textbf{Ours vs. end-to-end hair color control}}
\label{fig:end2end_hair}
\end{figure}

==> figures/fig_ours_vs_e2e_ori.tex <==
\begin{figure}[]
%\centering
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1}

\begin{tabular}{c}
    \footnotesize
    \hspace{4mm}\begin{tabularx}{0.9\linewidth}{ Y Y Y Y Y }
    Yaw=$0\degree$ Pitch=$0\degree$ &
    \hspace{2mm}$30\degree$ \newline $0\degree$ &
    $-30\degree$ \newline $0\degree$ &
    \hspace{2mm}$0\degree$ \newline $20\degree$ &
    \hspace{2mm}$0\degree$ \newline $-20\degree$
    \end{tabularx}
    \\
    \footnotesize
    % \hspace{4mm}\begin{tabularx}{0.9\linewidth}{ Y Y Y Y Y }
    % Pitch=$0\degree$ &
    % $0\degree$ &
    % $0\degree$ &
    % $20\degree$ &
    % $-20\degree$
    % \end{tabularx}
    % \\
    \rotatebox{90}{
    \begin{tabularx}{0.36\linewidth}{ Y }
        \footnotesize
        E2E
    \end{tabularx}}
    \includegraphics[width=0.9\linewidth]{images/end2end_comp/ori/e2e.jpg}
    \\
    \rotatebox{90}{
    \begin{tabularx}{0.36\linewidth}{ Y }
        \footnotesize
        E2E-10x
    \end{tabularx}}
    \includegraphics[width=0.9\linewidth]{images/end2end_comp/ori/e2e10x.jpg}
    \\
    \rotatebox{90}{
    \begin{tabularx}{0.36\linewidth}{ Y }
        \footnotesize
        \textbf{Ours}
    \end{tabularx}}
    \includegraphics[width=0.9\linewidth]{images/end2end_comp/ori/ours.jpg}
    \\
    
\end{tabular}

\caption{\textbf{Ours vs. end-to-end pose control}}
\label{fig:end2end_ori}
\end{figure}

==> figures/fig_r4_vs_ours_old.tex <==
\begin{figure}[htbp!]
\newcolumntype{Y}{>{\centering\arraybackslash}X}

\definecolor{color0}{rgb}{0.2181, 0.1311, 0.0883}
\definecolor{color1}{rgb}{0.7321048 , 0.6154765 , 0.36478823}

\setlength{\tabcolsep}{0pt}
\renewcommand{\arraystretch}{0}
\begin{tabular}{c}
    \tiny
    \begin{tabularx}{0.98\linewidth}{ Y Y Y Y Y Y }
    & 
    Yaw,Pitch$\!=\!0\degree$ Right side Illum. &
    \textcolor{color1}{\textbf{Hair color}} \linebreak Exp. 2 &
    Age$=\!45$yo \linebreak Exp. 3 & 
    Age$=\!75$yo \linebreak Front side Illum.&
    Yaw$\!=\!-30\degree$ Pitch$\!=\!0\degree$
    \end{tabularx}
    \\
    \includegraphics[width=0.98\linewidth]{iccv2021RebuttalKit/latex/images/r4/r4_00.jpg} \\
    \includegraphics[width=0.98\linewidth]{iccv2021RebuttalKit/latex/images/r4/r4_01.jpg} \\
    \includegraphics[width=0.98\linewidth]{iccv2021RebuttalKit/latex/images/r4/r4_02.jpg} \\
    \includegraphics[width=0.98\linewidth]{iccv2021RebuttalKit/latex/images/r4/r4_03.jpg} \\
    \includegraphics[width=0.98\linewidth]{iccv2021RebuttalKit/latex/images/r4/r4_04.jpg} \\
    \includegraphics[width=0.98\linewidth]{iccv2021RebuttalKit/latex/images/r4/r4_05.jpg} \\
    \includegraphics[width=0.98\linewidth]{iccv2021RebuttalKit/latex/images/r4/r4_06.jpg} \\
    \includegraphics[width=0.98\linewidth]{iccv2021RebuttalKit/latex/images/r4/r4_07.jpg} \\
    
    
\end{tabular}

\begin{tabular}{c}
    \includegraphics[width=0.98\linewidth]{iccv2021RebuttalKit/latex/images/ours/ours_00.jpg} \\
    \includegraphics[width=0.98\linewidth]{iccv2021RebuttalKit/latex/images/ours/ours_01.jpg} \\
    \includegraphics[width=0.98\linewidth]{iccv2021RebuttalKit/latex/images/ours/ours_02.jpg} \\
    \includegraphics[width=0.98\linewidth]{iccv2021RebuttalKit/latex/images/ours/ours_03.jpg} \\
    \includegraphics[width=0.98\linewidth]{iccv2021RebuttalKit/latex/images/ours/ours_04.jpg} \\
    \includegraphics[width=0.98\linewidth]{iccv2021RebuttalKit/latex/images/ours/ours_05.jpg} \\
    \includegraphics[width=0.98\linewidth]{iccv2021RebuttalKit/latex/images/ours/ours_06.jpg} \\
    \includegraphics[width=0.98\linewidth]{iccv2021RebuttalKit/latex/images/ours/ours_07.jpg} \\
    \includegraphics[width=0.98\linewidth]{iccv2021RebuttalKit/latex/images/ours/ours_10.jpg} 
    
\end{tabular}

\vspace{-0.2cm}
\tiny
\caption{\textbf{Suggestion vs. ours:} Every row is set to the the same ID, Left column attributes are set to: Yaw$\!=\!30\degree$, Pitch$\!=\!-15\degree$, Age$=\!25$yo, Exp. 1, \textcolor{color1}{\textbf{Hair color}} and Illum. 1. In each other column the above attributes are changed compered to the left column.}
\label{fig:r4_vs_ours}
\end{figure}

==> stylegan2_baseline.tex <==
\subsection{StyleGAN2 baseline}
\label{sec:ablation study}

As suggested by R4, we trained an attribute encoder using a pretrained StyleGAN2.
Since StyleGAN2's $\mathcal{W}$ is not divided into disentangled sub-spaces, we have to train a single encoder mapping all inputs (together) to $\mathcal{W}$. %the encoder must map all inputs (together) to $\mathcal{W}$.
The motivation for our design choices are simplicity, common sense and fair comparison.
The encoder ($E$) architecture consists of: $N$ per-attribute encoders and an ID encoder, concatenation and an aggregating encoder.
% The encoder architecture is as follows:
% First, each attribute is embedded using a per-attribute encoder.
% Then, all sub-encoders' output vectors are concatenated and passed through a single encoder.
When training, the inputs to $E$ are the predicted attributes and the ID (predicted ArcFace embedding vector). %where the ID input is the embedding vector predicted by ArcFace.
%$E$'s output is a $\mathbf{w}$ vector.
Table~\ref{tab:id_preservation} indicates that for this baseline ID is not preserved when the latent space is not disentangled.
%indicates that without a disentangled latent space the ID is not preserved.
%indicates that ID is not preserved when the latent space is not disentangled. without
This is also evident from the first row of Fig.~\ref{fig:r4_vs_ours}.
Table~\ref{tab:precision} demonstrates that the precision of the control is inferior except for expression.
% We hypothesize that control is partially achieved by ``adjusting the ID'' to match the desired attribute
We hypothesize that in order to reach a desired control, the model partially ``adjusts the ID''.
This is most prominent in expression where the geometry of the face changes.
Thus with limited ID preservation, it is ``easier'' to achieve a desired expression.
In Fig.~\ref{fig:r4_vs_ours} row 3 we show different images generated for different ID vectors but with the same set of controls.
This demonstrates that the entanglement limits the possible IDs, given a set of controls.

\input{figures/fig_r4_vs_ours_new.tex}
\input{tabels/table_id_preservation}
\input{tabels/table_control_percision}

==> tabels/table_control_percision.tex <==
\begin{table}[t]
    \setlength{\textwidth}{0pt}
    \newcolumntype{?}{!{\vrule width 1pt}}
    \centering
    \footnotesize
	\begin{tabular}{l?c|c|c}
    \toprule
	Control & Ours & R4 suggestion & FFHQ
	\\
    \hline
    Pose [$\degree$] $\downarrow$ & $\pmb{2.29}$\tiny{$\pmb{\pm1.31}$} & $5.44$\tiny{$\pm3.4$} & $23.8$\tiny{$\pm14.6$}\\
    Age [yo] $\downarrow$& $\pmb{2.02}$\tiny{$\pmb{\pm1.38}$} & $7.11$\tiny{$\pm6.1$} & $16.95$\tiny{$\pm12.9$}\\
    Exp. $\downarrow$ & $3.68$\tiny{$\pm0.7$} & $\pmb{2.94}$\tiny{$\pmb{\pm0.6}$} & $4.45$\tiny{$\pm0.9$}\\
    Illum. $\downarrow$ & $0.32$\tiny{$\pm0.13$} & $0.32$\tiny{$\pm0.14$} & $0.62$\tiny{$\pm0.2$}\\
    Hair color $\downarrow$ & $\pmb{0.13}$\tiny{$\pmb{\pm0.18}$} & $0.15$\tiny{$\pm0.14$} & 0.34\tiny{$\pm0.25$} \\
    \bottomrule
    \end{tabular}
    \vspace{-0.2cm}
    \caption{\textbf{Control precision$\downarrow$.} 
    % Same as Table 3 in the paper with R4 proposal.
    %Same as Table 3.
    }
    \label{tab:precision}
    %\setlength{\belowcaptionskip}{-50pt}
\end{table}

==> tabels/table_id_preservation.tex <==
\begin{table}[t]
    \setlength{\textwidth}{0pt}
    \newcolumntype{?}{!{\vrule width 1pt}}
    \centering
    \footnotesize
	\begin{tabular}{l?c|c|c}
    \toprule
	ID & Ours & R4 suggestion & FFHQ
	\\
    \hline
    Same$\downarrow$ & $\pmb{0.68}$\tiny{$\pmb{\pm0.19}$} & $1.16$\tiny{$\pm0.34$} & $1.89$\tiny{$\pm0.21$}
    \\
    Not same$\uparrow$ & $\pmb{1.9}$\tiny{$\pmb{\pm0.24}$} & $1.7$\tiny{$\pm0.26$} &  $1.89$\tiny{$\pm0.21$}
    \\
    \bottomrule
    \end{tabular}
    % \caption{\textbf{Identity preservation:} Same as Table 4 in the paper with R4 proposal.}
    \vspace{-0.2cm}
    \footnotesize
    \caption{\textbf{Identity preservation.}}
    \label{tab:id_preservation}
    %\setlength{\belowcaptionskip}{-50pt}
\end{table}

==> tabels/table_ours_vs_end2end.tex <==
\begin{table}[]
    \setlength{\textwidth}{0pt}
    \newcolumntype{?}{!{\vrule width 1pt}}
    \centering
    \small
	\begin{tabular}{l?c|c|c|c}
        \toprule
	     &  \textbf{Ours} &  E2E &  E2E-10x & FFHQ
	    \\
        \hline
        \multicolumn{5}{c}{\textbf{Control precision}}\\
        \hline
        Pose [$\degree$] & $\pmb{2.29}$\tiny{$\pmb{\pm1.31}$} & $10.35$\tiny{$\pm7.8$} & $4.36$\tiny{$\pm0.82$} & $23.8$\tiny{$\pm15$}\\
        Age [yo]& $\pmb{2.02}$\tiny{$\pmb{\pm1.38}$} & $14.63$\tiny{$\pm8.4$} & $14.38$\tiny{$\pm8.5$} & $16.95$\tiny{$\pm13$}\\
        Exp. & $\pmb{3.68}$\tiny{$\pmb{\pm0.7}$} & $4.41$\tiny{$\pm0.8$}  & $4.36$\tiny{$\pm0.8$} & $4.45$\tiny{$\pm0.9$}\\
        Illum. & $\pmb{0.32}$\tiny{$\pmb{\pm0.13}$} & $0.62$\tiny{$\pm0.21$} & $0.61$\tiny{$\pm0.21$} & $0.62$\tiny{$\pm0.2$}\\
        Hair c. & $\pmb{0.13}$\tiny{$\pmb{\pm0.18}$} & $0.33$\tiny{$\pm0.24$} & $0.24$\tiny{$\pm0.18$} & 0.34\tiny{$\pm0.25$} \\
        \hline
        \multicolumn{5}{c}{\textbf{ID preservation}}\\
        \hline
        Same$\downarrow$ & 
        $\pmb{0.68}$\tiny{$\pmb{\pm0.19}$} & 
        $0.82$\tiny{$\pm0.3$} & 
        $0.97$\tiny{$\pm0.35$} & 
        $1.89$\tiny{$\pm0.21$}
        \\
        Not same$\uparrow$ & 
        $\pmb{1.9}$\tiny{$\pmb{\pm0.24}$} &
        $1.78$\tiny{$\pm0.23$} & 
        $1.79$\tiny{$\pm0.25$} & 
        $1.89$\tiny{$\pm0.21$}
        \\
        \hline
        \multicolumn{5}{c}{\textbf{FID}} \\
        \hline
        FID$\downarrow$ & $\pmb{5.72}$ & $6.48$ & $9.1$ &\\
        \bottomrule
    \end{tabular}
    \caption{\textbf{Ours vs. end-to-end training comparison}}
    \label{tab:table_end2end}
\end{table}
